Stochastic Matching with Few Queries: New Algorithms and Tools

We consider the following stochastic matching problem on both weighted and unweighted graphs: A graph $G(V, E)$ along with a parameter $p \in (0, 1)$ is given in the input. Each edge of $G$ is realized independently with probability $p$. The goal is to select a degree bounded (dependent only on $p$) subgraph $H$ of $G$ such that the expected size/weight of maximum realized matching of $H$ is close to that of $G$. This model of stochastic matching has attracted significant attention over the recent years due to its various applications. The most fundamental open question is the best approximation factor achievable for such algorithms that, in the literature, are referred to as non-adaptive algorithms. Prior work has identified breaking (near) half-approximation as a barrier for both weighted and unweighted graphs. Our main results are as follows: -- We analyze a simple and clean algorithm and show that for unweighted graphs, it finds an (almost) $4\sqrt{2}-5$ ($\approx 0.6568$) approximation by querying $O(\frac{\log (1/p)}{p})$ edges per vertex. This improves over the state-of-the-art $0.5001$ approximate algorithm of Assadi et al. [EC'17]. -- We show that the same algorithm achieves a $0.501$ approximation for weighted graphs by querying $O(\frac{\log (1/p)}{p})$ edges per vertex. This is the first algorithm to break $0.5$ approximation barrier for weighted graphs. It also improves the per-vertex queries of the state-of-the-art by Yamaguchi and Maehara [SODA'18] and Behnezhad and Reyhani [EC'18]. Our algorithms are fundamentally different from prior works, yet are very simple and natural. For the analysis, we introduce a number of procedures that construct heavy fractional matchings. We consider the new algorithms and our analytical tools to be the main contributions of this paper.

==> adaptive.tex <==
\section{Our Adaptive Algorithm}
In this section we give an adaptive algorithm for both weighted and unweighted graphs that in $1/\epsilon$ rounds finds a $1-\epsilon$ approximation.

The algorithm --- formalized as Algorithm~\ref{alg:adaptive} --- in each round of adaptivity takes $R^\star$ independent random realizations of the graph and queries the edges in maximum weighted matching of each of these realizations simultaneously. Each round of the algorithm is similar to our non-adaptive algorithm (Algorithm~\ref{alg:nonadaptive}). The only difference is that after each round, we remove all of the unrealized edges from $E$, and we enforce the edges that we already know are realized to appear in all random realizations that we take.

\begin{algorithm}
  \caption{An adaptive algorithm for the weighted stochastic matching problem.}
  \label{alg:adaptive}
  \begin{algorithmic}[1]
  	\Statex \textbf{Input:} Input graph $G=(V, E)$, edge weights $w: E \to \mathbb{R}_+$ and realization probability $p \in [0, 1]$.
  	\Statex \textbf{Parameters:} $R=1/\epsilon$ and $R^\star = O(\frac{\log(1/\epsilon p)}{\epsilon^3 p})$.
  	\State $P_1 \gets \emptyset$ \Comment{$P_i$ denotes the set of edges that we know are realized at the start of round $i$.}
  	\State $E^\star \gets E$
  	\For{$r= 1, \ldots, R$}\Comment{Rounds of adaptivity.}
  	\State $P_{r+1} \gets P_r$
  	\State $S_r \gets \emptyset$
	\For{$r^\star = 1, \ldots, R^\star$}\Comment{Process of constructing our sample for this round.}
		\State Construct a realization $\mathcal{G}_{r^\star}=(V, \mathcal{E}_{r^\star})$ of $G$, where any edge $e \in (E^\star \setminus S)$ appears in $\mathcal{E}_{r^\star}$ independently with probability $p$, and each edge in $P_r$ appears with probability $1$.
		\State Add the edges in maximum weighted matching $\matching{\mathcal{E}_{r^\star}}$ of $\mathcal{G}_{r^\star}$ to $S_r$.
	\EndFor
		\State Query the edges in $S_r$.
		\State Remove unrealized edges from $E^\star$, and add realized edges to $P_r+1$.
	\EndFor
  \State Return the maximum weighted matching of $P_{R+1}$.

  \end{algorithmic}
\end{algorithm}

We need a few definitions before the analysis. At the beginning of round $r$, for each edge $e \in E$, we define $q^r_e$ to be the probability that edge $e$ appears in the omniscient optimum matching given the realizations by round $r-1$. Let $C_r := \{e \, | \, q^r_e \geq \tau \}$ and $N_r := \{ e \, | \, q^r_e < \tau \}$ respectively denote the crucial and non-crucial edges at the beginning of the round $r$ where $\tau$ is asymptotically the same threshold used in the previous section (we soon mention a slight change in the constant factor of this threshold). Moreover, for any $r$ denote $\qw^r_e := q^r_e \cdot w_e$. We need one more definition to continue. Define $$Z_i = \expm \Big( E \, |\, \text{given the outcome of our queries by round $i-1$} \Big).$$
Note that with this definition we have $Z_1 = \opt$ and $\qw^r(E) = Z_r$ for any $r$. In the following claim, we show that if  $q^r(C_r \setminus S_r)$ is at most $\sfrac{\epsilon}{2} \cdot \opt$, then the expected weight of the maximum realized matching found by the end of round $r$ is at least $(1-\epsilon) Z_r$.

\begin{lemma}
	$\E_{r}[\qw^{r+1}(P_{r+1})] \geq (1-\epsilon)\qw^{r}(P_{r}) + \epsilon \cdot \qw^r(E)$.
\end{lemma}
\begin{proof}
	We assume that we are at the beginning of round $r$ and argue that $\E_{r}[\qw^{r+1}(P_{r+1})]$ is large. Let us consider the following inequality which is equivalent to our desired bound
	$$\E_r[\qw^{r+1}(P_{r+1})] - \qw^{r}(P_{r}) \geq \epsilon\big(\qw^r(E) - \qw^{r}(P_{r})\big).$$
	Note that $P_{r+1}$, the set of edges realized by the end of round $r$, is a random variable whose value is determined at the end of our current round $r$. We consider two scenarios. First, assume that the expected matching of un-queried crucial edges is {\em large}. More precisely, suppose $\qw^r(C_r \setminus P_r) \geq \sfrac{\epsilon}{2} \cdot \qw^r(E)$. In this case, as shown by Lemma~\ref{lem:sampleallcrucial}, we expect our algorithm to query a subset $Z_r \subseteq C_r \setminus P_r$ of these crucial edges where $\E_r[\qw^r(Z_r)] \geq (1-\epsilon)\qw^r(C_r \setminus P_r)$. This means that we have 
	$$\E_r[\qw^r(P_r \cup Z_r)] = \qw^r(P_r) + \E_r[\qw^r(Z_r)] \geq \qw^r(P_r) + \frac{(1-\epsilon)\epsilon}{2} \cdot \qw^r(E).$$
	Furthermore, one can easily verify that $\E_r[\qw^{r+1}(P_{r+1})] \geq \E_r[\qw^r(P_r \cup Z_r)]$. The reason is that every realized edge in $P_r \cup Z_r$ also appears.
	
	
	$$\E_r[\qw^{r+1}(P_{r+1})] - \qw^{r}(P_r) \geq \qw^r(C_r \setminus P_r) \geq (1-\epsilon) \frac{(1-\epsilon)\epsilon}{2} \cdot \qw^r(E)$$
	as desired.
\end{proof}

\begin{claim}
Suppose that in a round $r$ of the algorithm, the expected matching of unrealized crucial edges is most $\sfrac{\epsilon}{2} \cdot \opt$, i.e., $q^r(C_r \setminus S_r) \le \sfrac{\epsilon}{2} \cdot \opt$. Then the expected weight of the matching returned by the algorithm during this round is at least $(1-10\epsilon) \opt$.
\end{claim} 
\begin{proof}
Let $N'$ (resp. $C'$) be the set of non-crucial (crucial) edges which are not known to be realized yet, i.e., they are not in $S_r$. Then, we have $\opt \le \qw(N')+ \qw(S_r) + \qw(C')$. We run Procedure \ref{proc:non-crucial} on the realized edges of $N'$ in $Q_r$. Let $x^{N'}$ be the fractional matching obtained by the procedure. By Lemma~\ref{lem:non-cruciallemma}, we have
$$
\E\bigg[\sum_{e \in S_{r+1} \cap N'} x^{N'}_e \cdot w_e \bigg]\geq (1-9\epsilon) \qw(N') \,.
$$
However, we can assume at the cost of a constant factor more per-vertex queries for each round (more precisely by changing the threshold for crucial/non-crucial edges) that:
$$
\E\bigg[\sum_{e \in S_{r+1} \cap N'} x^{N'}_e \cdot w_e \bigg]\geq (1-\epsilon/2) \qw(N') \,.
$$

For each edge $e$ in $S_r$, we add $e$ to our fractional matching and set $x_e = (1-\epsilon/2) q(e)$. For every edge $e$ in $N'$, we set $x_e = x^{N'}_e$. Then we have
$$
\E\bigg[\sum_{e \in S_r \cup ( S_{r+1} \cap N')} x_e \cdot w_e \bigg]\geq (1-\epsilon/2) \qw(S_r)+  (1-\epsilon/2) \qw(N') = (1-\epsilon/2)\big( \qw(S_r) + \qw(N') \big)\,.
$$
Since $\qw(C') \le \sfrac{\epsilon}{2} \cdot \opt$, we have
$$
\E\bigg[\sum_{e \in S_r \cup ( S_{r+1} \cap N')} x_e \cdot w_e \bigg]\geq \qw(S_r)+  (1-\epsilon/2) \qw(N') \ge (1-\epsilon) \opt \,.
$$
\end{proof}
\begin{theorem}\label{thm:adaptive}
For any graph $G$, the expected weight of the matching returned by Algorithm \ref{alg:adaptive} is at least $(1-\epsilon) \opt$.
\end{theorem}

